Information Leakage through Physical Layer Supply Voltage Coupling Vulnerability

Side-channel attacks exploit variations in non-functional behaviors to expose sensitive information across security boundaries. Existing methods leverage side-channels based on power consumption, electromagnetic radiation, silicon substrate coupling, and channels created by malicious implants. Power-based side-channel attacks are widely known for extracting information from data processed within a device while assuming that an attacker has physical access or the ability to modify the device. In this paper, we introduce a novel side-channel vulnerability that leaks data-dependent power variations through physical layer supply voltage coupling (PSVC). Unlike traditional power side-channel attacks, the proposed vulnerability allows an adversary to mount an attack and extract information without modifying the device. We assess the effectiveness of PSVC vulnerability through three case studies, demonstrating several end-to-end attacks on general-purpose microcontrollers with varying adversary capabilities. These case studies provide evidence for the existence of PSVC vulnerability, its applicability for on-chip as well as on-board side-channel attacks, and how it can eliminate the need for physical access to the target device, making it applicable to any off-the-shelf hardware. Our experiments also reveal that designing devices to operate at the lowest operational voltage significantly reduces the risk of PSVC side-channel vulnerability.

==> fig/kb2.tex <==
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte0_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 0}\label{lst:appteplate}
\end{subfigure}%
% \hspace{-1em}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte1_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 1}\label{lst:wrapper}
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte2_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 2}\label{lst:wrapper}
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte3_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 3}\label{lst:wrapper}
\end{subfigure}

\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte4_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 4}\label{lst:appteplate}
\end{subfigure}%
% \hspace{-1em}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte5_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 5}\label{lst:wrapper}
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte6_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 6}\label{lst:wrapper}
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte7_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 7}\label{lst:wrapper}
\end{subfigure}


\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte8_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 8}\label{lst:appteplate}
\end{subfigure}%
% \hspace{-1em}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte9_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 9}\label{lst:wrapper}
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte10_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 10}\label{lst:wrapper}
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte11_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 11}\label{lst:wrapper}
\end{subfigure}

\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte12_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 12}\label{lst:appteplate}
\end{subfigure}%
% \hspace{-1em}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte13_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 13}\label{lst:wrapper}
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte14_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 14}\label{lst:wrapper}
\end{subfigure}
\hspace{-0.1in}
\begin{subfigure}{.25\linewidth}
\begin{center}
% \vspace{-0.1in}
\includesvg[width=\textwidth]{fig/byte15_corr_coef_with_num_traces.svg}
\end{center}
\vspace{-0.2in}
\caption{Byte 15}\label{lst:wrapper}
\end{subfigure}
